Th\'eor\`emes d'\'equidistribution pour les syst\`emes dynamiques d'origine arithm\'etique

This survey article is about algebraic dynamics. It is mainly concerned by the arithmetic equidistribution theorems featured by dynamical systems. The contents are: - heights - algebraic dynamics, conjectures - equidistribution theorem on the projective line (after Bilu and Baker). It was written for the sesion 2006 of \'Etats de la recherche, Syst\`emes dynamiques polynomiaux.

==> frenchbst.tex <==
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{\'editeurs}        \def\bbleds{\'eds.}
\def\bbleditor{\'editeur}          \def\bbled{\'ed.}
\def\bbledby{\'edit\'e by}
\def\bbledition{\'edition}        \def\bbledn{\'ed.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n\textsuperscript o}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{p.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Pr\'epublication}
\def\bbltechrep{Pr\'ep.}
\def\bblmthesis{M\'emoire de DEA}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1\textsuperscript{re}}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\textsuperscript{e}}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\textsuperscript{e}}
\def\bblfourth{Fourth}          \def\bblfourtho{4\textsuperscript{e}}
\def\bblfifth{Fifth}            \def\bblfiftho{5\textsuperscript{e}}
\def\bblst{\textsuperscript{re}}
  \def\bblnd{\textsuperscript{e}}  \def\bblrd{\textsuperscript{e}}
\def\bblth{\textsperscript{e}}
\def\bbljan{Janvier}  \def\bblfeb{F\'evrier}  \def\bblmar{Mars}
\def\bblapr{Avril}    \def\bblmay{Mai}       \def\bbljun{Juin}
\def\bbljul{Juillet}     \def\bblaug{Ao\^ut}    \def\bblsep{Septembre}
\def\bbloct{Octobre}  \def\bblnov{Novembre}  \def\bbldec{Decembre}


